DMKD: Improving Feature-based Knowledge Distillation for Object Detection Via Dual Masking Augmentation

Recent mainstream masked distillation methods function by reconstructing selectively masked areas of a student network from the feature map of its teacher counterpart. In these methods, the masked regions need to be properly selected, such that reconstructed features encode sufficient discrimination and representation capability like the teacher feature. However, previous masked distillation methods only focus on spatial masking, making the resulting masked areas biased towards spatial importance without encoding informative channel clues. In this study, we devise a Dual Masked Knowledge Distillation (DMKD) framework which can capture both spatially important and channel-wise informative clues for comprehensive masked feature reconstruction. More specifically, we employ dual attention mechanism for guiding the respective masking branches, leading to reconstructed feature encoding dual significance. Furthermore, fusing the reconstructed features is achieved by self-adjustable weighting strategy for effective feature distillation. Our experiments on object detection task demonstrate that the student networks achieve performance gains of 4.1% and 4.3% with the help of our method when RetinaNet and Cascade Mask R-CNN are respectively used as the teacher networks, while outperforming the other state-of-the-art distillation methods.

==> relate.tex <==
\section{Related Work}
In this section, we comprehensively review the recent advance in object detection and knowledge distillation, both of which are closely related to our method.
\subsection{Object Detection}
Object detection, as a foundational task in computer vision, is dedicated to identifying both the category and precise location of objects within an image. In recent times, the remarkable strides made by Convolutional Neural Networks (CNNs) have propelled the field of object detection to new heights. Broadly speaking, object detectors utilizing deep CNN architectures can be categorized into three distinct groups: anchor-based detectors \cite{ren2015faster,fu2017dssd}, anchor-free detectors \cite{tian2019fcos}, and end-to-end detectors \cite{carion2020end}.
In particular, anchor-based detection models are divided into two-stage \cite{gidaris2015object,ren2015faster,kong2016hypernet,he2017mask} and one-stage detectors \cite{redmon2018yolov3,ge2021yolox,fu2017dssd}.
The previous approach to detection, exemplified by algorithms like R-CNN \cite{girshick2015fast,ren2015faster}, boasts superior detection accuracy. However, its inference speed often falls short of expectations due to the resource-intensive nature of the region proposal network (RPN), leading to impracticality in real-time scenarios. On the other hand, one-stage detectors take a different approach by directly executing classification and regression on anchors, eliminating the need for preliminary proposal generation. Consequently, these detectors offer faster processing while maintaining an assured level of detection performance.

\subsection{Knowledge Distillation}
Knowledge distillation is gaining traction in model compression due to its ability to maintain compact models with improved performance. Hinton et al. \cite{hinton2015distilling} pioneered this concept, integrating soft labels from the teacher network into the student network's loss function. This enables the student network to learn the teacher model's probability distribution fitting, particularly valuable for classification tasks.
Chen et al. \cite{chen2017learning} distilled the neck feature, classification head, and regression head by setting up three loss functions, respectively.
Li et al. \cite{li2017mimicking} used region proposals of the larger network to help the smaller network learn higher semantic information. 
Shu et al. \cite{shu2021channel} propose to minimize the Kullback-Leibler (KL) divergence of the corresponding channels of the two networks. 
Yang et al. \cite{yang2022masked} applies random masking to the student model's feature map, leading to the generation of a reconstructed feature map from the teacher network.
Yang et al. \cite{yang2023amd} performed attention-guided spatial masking instead of random masking on the feature map of the student network,  such that we can identify the important
features via spatially adaptive feature masking.







